Undesignable RNA Structure Identification via Rival Structure Generation and Structure Decomposition

RNA design is the search for a sequence or set of sequences that will fold into predefined structures, also known as the inverse problem of RNA folding. While numerous RNA design methods have been invented to find sequences capable of folding into a target structure, little attention has been given to the identification of undesignable structures according to the minimum free energy (MFE) criterion under the Turner model. In this paper, we address this gap by first introducing mathematical theorems outlining sufficient conditions for recognizing undesignable structures, then proposing efficient algorithms, guided by these theorems, to verify the undesignability of RNA structures. Through the application of these theorems and algorithms to the Eterna100 puzzles, we demonstrate the ability to efficiently establish that 15 of the puzzles indeed fall within the category of undesignable structures. In addition, we provide specific insights from the study of undesignability, in the hope that it will enable more understanding of RNA folding and RNA design.

==> Makefile <==
texbin=/Library/TeX/texbin
#texbin=/usr/local/texlive/2018/bin/x86_64-darwin
main:
	rm -rf *.run.xml *.bcf *.aux *.out *.blg *.bbl *.log *.fls *.fdb_latexmk *~
	${texbin}/pdflatex main
	${texbin}/bibtex main
	if ${texbin}/bibtex siref; then \
		echo "seperate references\n"; \
	else \
		echo "combined references\n"; \
	fi
	${texbin}/pdflatex main
	${texbin}/pdflatex main
# supp:
# 	rm -rf *.run.xml *.bcf *.aux *.out *.blg *.bbl *.log *.fls *.fdb_latexmk *~
# 	${texbin}/pdflatex supp
# 	${texbin}/pdflatex supp       
split:
	yes | gs -dBATCH -sOutputFile="main.submit.pdf" -dFirstPage=1 -dLastPage=13 -sDEVICE=pdfwrite main.pdf 
	yes | gs -dBATCH -sOutputFile="supp.pdf" -dFirstPage=14 -dAutoRotatePages=/None -sDEVICE=pdfwrite main.pdf  

clean:
	rm -rf  *.run.xml *.bcf *.bbl *.xwm *.aux *.out *.blg *.log *.fls *.fdb_latexmk main.pdf *~ 

fast:
	${texbin}/pdflatex main


